Valinor: Architectural Support for Fast, Energy-Efficient and Programmable Physical Memory Allocation

Physical memory allocation establishes virtual-to-physical mappings on demand. In current systems, each minor page fault traps into the kernel and triggers pipeline flushes, stalls, and a long sequence of allocation steps that can cost tens of thousands of cycles. These overheads are increasingly significant for short-lived workloads such as serverless functions and microservices, where minor faults can account for up to 54% of runtime and up to 40% of system energy. Prior hardware allocation proposals avoid traps and context switches, but either sacrifice useful placement optimizations or rely on fixed-function logic that cannot adapt to new policies or changing hardware conditions. We present Valinor, a hardware-OS cooperative memory allocation substrate that combines software flexibility with hardware-class performance. Valinor introduces a programmable hardware allocation engine that executes compact OS-supplied allocation libraries at close to fixed-hardware speed. It supports diverse policies, including short-lived object allocators, integrity mechanisms, and hardware-telemetry-guided placement. We implement Valinor on a BOOM RISC-V soft core running Linux and in a full-system simulator. On real hardware, Valinor accelerates allocation by 17x, improves end-to-end performance by 16%, and reduces energy consumption by up to 8%. Full-system simulation further evaluates the programmable allocation engine and six allocation libraries, showing that Valinor provides hardware-class performance without sacrificing programmability.

==> tables/libraries.tex <==
\begin{table*}[bh!]
\centering
\footnotesize
\renewcommand{\arraystretch}{1.20}
\setlength{\tabcolsep}{5pt}

% Thick rules


\begin{tabular}{|p{2.3cm}|p{3.6cm}|p{3.8cm}|p{3.4cm}|p{2.8cm}|}
\toprule
\textbf{Name} & \textbf{Summary} & \textbf{Allocation Routine} & \textbf{Translation Routine} & \textbf{OS Sync} \\
\bottomrule

\textbf{Low-latency} &
Fast-path allocation for short-lived objects; optimized tail latency. &
Set-associative memory segment for quick allocation. &
Hash-based translation on PTW miss. &
Large region allocated at first use. \\
\hline

\textbf{Runahead} &
Hides allocation stalls using asynchronous pre-allocation. &
Background allocator fills a free-page pool; foreground allocates from it. &
Secondary page-table for pre-allocated pages. &
Pool growth triggers OS sync. \\
\hline

\textbf{Real-time} &
Provides deterministic bounded worst-case allocation latency. &
Allocates from pre-reserved contiguous region in a linear fashion. &
Offset-based translation. &
Rare sync for region exhaustion. \\
\hline

\textbf{Energy-efficient} &
Minimizes energy via low-frequency (i.e., PAE is downscaled by 50\%) background allocation. &
Background allocator replenishes free-page pool. &
Dedicated page-table for pooled pages. &
Rare sync for pool resizing. \\
\hline

\textbf{Rowhammer-safe} &
Inserts guard rows to mitigate Rowhammer. &
Page coloring enforces spacing constraints. &
Color-aware lookup on PTW miss. &
Single region allocated at boot. \\
\hline

\textbf{Integrity-enforcing} &
Adds integrity metadata (Merkle-tree) to protect mappings. &
Allocates pages with integrity tags in reserved space. &
Verifies integrity during translation. &
Requests segments to guarantee full coverage. \\
\hline

\textbf{Telemetry-aware} &
Adapts placement using hardware metrics (bank conflicts, bandwidth). &
Bank-level free lists; telemetry-guided placement. &
Bank-aware translation path. &
Large region allocated at first use. \\
\hline


\textbf{Shadow paging} &
Accelerates shadow page-table construction and translation in VMs. &
Allocates shadow PTEs from reserved region. &
Fast shadow page table walk. &
Requests segments for Shadow PT expansion. \\
\bottomrule

\end{tabular}

\caption{Example allocation libraries supported by Valinor’s programmable allocation engine.}
\label{tab:valinor_libraries}
\end{table*}

